Runtime Analysis of the $(1+(\lambda,\lambda))$ Genetic Algorithm on Random Satisfiable 3-CNF Formulas

The $(1+(\lambda,\lambda))$ genetic algorithm, first proposed at GECCO 2013, showed a surprisingly good performance on so me optimization problems. The theoretical analysis so far was restricted to the OneMax test function, where this GA profited from the perfect fitness-distance correlation. In this work, we conduct a rigorous runtime analysis of this GA on random 3-SAT instances in the planted solution model having at least logarithmic average degree, which are known to have a weaker fitness distance correlation. We prove that this GA with fixed not too large population size again obtains runtimes better than $\Theta(n \log n)$, which is a lower bound for most evolutionary algorithms on pseudo-Boolean problems with unique optimum. However, the self-adjusting version of the GA risks reaching population sizes at which the intermediate selection of the GA, due to the weaker fitness-distance correlation, is not able to distinguish a profitable offspring from others. We show that this problem can be overcome by equipping the self-adjusting GA with an upper limit for the population size. Apart from sparse instances, this limit can be chosen in a way that the asymptotic performance does not worsen compared to the idealistic OneMax case. Overall, this work shows that the $(1+(\lambda,\lambda))$ GA can provably have a good performance on combinatorial search and optimization problems also in the presence of a weaker fitness-distance correlation.

==> parts/__old-theorem-1.tex <==
The following theorem summarizes these ideas.

\begin{theorem}\label{3cnf-bounding-theorem}
Consider solving random 3-CNF formulas with planted solutions on $n$ variables and $m$ clauses by the $\onell$~GA, where $m / n > c \log n$ for large enough constant $c$. If there exists some $\lambdabound = o((m / n)^{1/4})$ such that, during the entire run of the $\onell$~GA, $\lambda \le \lambdabound$, and the algorithm starts at the distance of \revisepar{$(1/2 + \varepsilon) n$}{Reviewer~1 asked to elaborate on why the algorithm never drops beyond.} from the optimum, then with probability $1 - o(1)$, taken both over the random 3-CNF formulas and the algorithm decisions, the algorithm will demonstrate, in every point, the same progress, divided by at most constant, as the same algorithm optimising \textsc{OneMax} on $n$ variables.
\end{theorem}

\begin{proof}
Without loss of generality, we assume $\lambdabound$ is integer, and we fix the planted solution to all ones: $x^{*} = 11\ldots1$. In this proof, we treat the formula clauses $C_1, \ldots, C_m$, as well as the formula $F = \{ C_1, \ldots, C_m \}$ itself, as random variables, keeping in mind that every clause should be satisfiable by $x^{*}$. By $f(x)$ we denote a random variable which equals the number of clauses in $F$ satisfied by the assignment $x$. Recall also that $d(x)$ is the Hamming distance of the assignment $x$ to the planted solution.

Consider a fixed non-optimal assignment $x$, and a fixed mutation strength $\ell$. We define by $X^{-}$ the set of all \emph{bad} offspring of $x$, that is, the offspring $x'$ which have $d(x') = d(x) + \ell$ after applying a mutation which flips $\ell$ random bits. The set $X^{+}$ is the set of all \emph{good} offspring of $x$, that is, the offspring $x'$ which have exactly one of the bits missing in $x$ flipped,
and thus $d(x') = d(x) + \ell - 2$. All remaining offspring have more than one missing bits flipped, so we call a set of these offspring $X^{*}$ \emph{excellent}. Note that these sets depend exclusively on $x$, and they do not depend on the formula $F$.

Let $x^{-} \in X^{-}$ be a \emph{bad} offspring, and $f_{\avg}(x^{-})$ be its fitness averaged over all possible values of $F$. As all $x^{-} \in X^{-}$ have the same Hamming distance to the optimum, this average fitness is the same for all of them. This means we can introduce $f^{-} = f_{\avg}(x^{-})$ which does not depend on the actual $x^{-}$ chosen. Using similar arguments, we also introduce $f^{+}$, the average (over formulas $F$) fitness of every \emph{good} offspring. We also define the \emph{threshold} value $f^{=} = (f^{+} + f^{-}) / 2$.

A change in one bit of any assignment introduces a $\Theta(m / n)$ change in the fitness of this assignment, averaged over all $F$, so it holds that $f(x) - f^{-} = \Theta(m \ell / n)$ and $f^{+} - f^{-} = \Theta(m / n)$, as well as $f^{=} - f^{-} = \Theta(m / n)$.

\begin{definition}
An $x$ is \emph{well-behaved} for a formula $F$, iff:
\begin{itemize}
    \item in $X^{-}$ there are at most $|X^{-}|/\lambdabound$ members $x^{-}$ such that $f(x^{-}) \ge f^{=}$;
    \item in $X^{+}$ there are at most $|X^{+}| / 2$  members $x^{+}$ such that $f(x^{+}) \le f^{=}$;
    \item in $X^{*}$ there are at most $|X^{*}| / 2$  members $x^{*}$ such that $f(x^{*}) \le f^{=}$.
\end{itemize}
\end{definition}

We need the concept of being \emph{well-behaved} for the following lemma.

\begin{lemma}\label{ok-lemma}
Assume $x$ is the current best solution of the $\onell$~GA, and this $x$ is \emph{well-behaved}. Then, with at least constant probability, whenever at least one \emph{good} or \emph{excellent} offspring
appears at the mutation phase, the $\onell$~GA will choose one of them when taking the offspring with
the best fitness value.
\end{lemma}

\begin{proof}
Assume that, in the current step, $\ell$ was sampled from $\mathcal{B}(n, \lambda / n)$ in such a way
that $\ell \le \lambdabound$. As the median of $\mathcal{B}(n, \lambda / n)$ is at most $\lceil \lambda \rceil$, and $\lceil \lambda \rceil \le \lambdabound$, this happens with probability of at least $1/2$.

Assume $g \ge 1$ \emph{good} or \emph{excellent} offspring have been sampled, as well as $\ell - g$ \emph{bad} offspring. The probability of all \emph{bad} offspring to have a fitness value below the threshold is:
\begin{equation*}
\left(1 - \frac{1}{\lambdabound}\right)^{\ell - g} \ge \left(1 - \frac{1}{\lambdabound}\right)^{{\lambdabound} - 1} \ge e^{-1}.
\end{equation*}
The probability of, say, the first \emph{good} or \emph{excellent} offspring to have a fitness value above the threshold is at least $1/2$. Thus, the probability of the $\onell$~GA to choose an offspring which is not \emph{bad}, whenever it exists, is at least $e^{-1} / 4$.
\end{proof}

Note that Lemma~\ref{ok-lemma} enables us to assume, in the rest of the proof, that $\ell \le \lambdabound$, in particular, $\ell = O(\lambdabound)$.

Now we need to show that, under the conditions of this theorem, every $x$ is \emph{well-behaved} with an overwhelming probability. Recall that $f(x^{-})$, for $x^{-} \in X^{-}$, is a random variable which depends on $F$. We construct an indicator random variable $V(x^{-})$, such that
\begin{equation*}
V(x^{-}) = \begin{cases}
    1, & f(x^{-}) \ge f^{=}; \\
    0, & \text{otherwise}.
\end{cases}
\end{equation*}

We want to prove the following statement, which is equivalent to proving that the first part of the definition of $x$ being \emph{well-behaved} is violated with exponentially decreasing probability
\begin{equation}
\Pr\left[\sum_{x^{-} \in X^{-}} V(x^{-}) > \frac{|X^{-}|}{\lambdabound}\right] < e^{-\omega(n)}. \label{x-is-okay-part1}
\end{equation}

This expression calls for one of the Chernoff bounds to be applied. However, the resulting bounds are not strong enough for our aim to be achieved. Instead, we introduce a new random variable, $\tilde{V}(x^{-})$. Let $f^{\equiv} = (f^{-} + f^{=}) / 2$. Then
\begin{equation*}
\tilde{V}(x^{-}) = \begin{cases}
    0, & f(x^{-}) \le f^{\equiv}; \\
    (f(x^{-}) - f^{\equiv}) / (f^{=} - f^{\equiv}), & f^{\equiv} \le f(x^{-}) \le f^{=}; \\
    1, & f(x^{-}) \ge f^{=}.
\end{cases}
\end{equation*}

In simple words, $\tilde{V}(x^{-})$ starts growing linearly when $f(x^{-})$ is halfway from $f^{-}$ to $f^{=}$. As $\tilde{V}(x^{-}) \ge V(x^{-})$ with probability one, it is enough to show, instead of~\eqref{x-is-okay-part1}, that
\begin{equation}
\Pr\left[\sum_{x^{-} \in X^{-}} \tilde{V}(x^{-}) > \frac{|X^{-}|}{\lambdabound}\right] < e^{-\omega(n)}. \label{x-is-okay-part1-tilde}
\end{equation}

We denote for brevity $\tilde{V}^{\Sigma} = \sum_{x^{-} \in X^{-}} \tilde{V}(x^{-})$. We interpret the random variable $\tilde{V}^{\Sigma}$ as a function of independent random variables $C_1, \ldots, C_m$ which represent clauses. A different sampling of a single $C_i$ introduces a change of at most $2 / (f^{=} - f^{\equiv}) = \Theta(n / m)$ in the $\tilde V$ value of every $x^{-}$ which are influenced by this change. There are at most $\binom{n - d}{\ell} - \binom{n - d - 6}{\ell} = \sum_{i=0}^5 \left(\binom{n-d-i}{\ell} - \binom{n-d-(i+1)}{\ell}\right) = \sum_{i=0}^5 \binom{n-d-(i+1)}{\ell-1} \le 6 \binom{n-d-1}{\ell-1} = 6 \binom{n - d}{\ell} \frac{\ell}{n - d} = |X^{-}| \cdot\Theta(\ell / n)$ such $x^{-}$, where $d = d(x)$ is the Hamming distance of $x$ to the optimum. The total change of $\tilde{V}^{\Sigma}$, when one of the clauses changes, is thus $|X^{-}| \cdot O(\ell / m)$.

We use the latter statement to apply the McDiarmid's inequality, see~\eqref{mcdiarmid-ge}, and obtain
\begin{align}
\Pr\left[\tilde{V}^{\Sigma} > |X^{-}| / \lambdabound\right]
  &= \Pr\left[\tilde{V}^{\Sigma} > E\left[\tilde{V}^{\Sigma}\right] + \left(|X^{-}| / \lambdabound - E\left[\tilde{V}^{\Sigma}\right]\right)\right] \nonumber\\
  &\le \exp\left(-\frac{2\left(|X^{-}| / \lambdabound - E\left[\tilde{V}^{\Sigma}\right]\right)^2}{m \cdot (|X^{-}| \cdot O(\ell / m))^2}\right) \nonumber\\
  &=   \exp\left(-\Omega\left(\frac{m \cdot \left(1 - \lambdabound \frac{E[\tilde{V}^{\Sigma}]}{|X^{-}|}\right)^2}{\ell^2 \lambdaboundsq}\right)\right). \label{failure-prob-raw}
\end{align}

To complete this bound, we need to show that the term $(1 - \lambdabound E[\tilde{V}^{\Sigma}] / |X^{-}|)$ is at least some positive constant. To do this with the least effort, we introduce the random variable $\overline{V}(x^{-})$ defined by 
\begin{equation*}
\overline{V}(x^{-}) = \begin{cases}
    1, & f(x^{-}) \ge f^{\equiv}, \\
    0, & \text{otherwise}
\end{cases}
\end{equation*}
for all $x^{-} \in X^-$, and observe that it dominates $\tilde{V}(x^{-})$. Consequently, we have $E[\tilde{V}(x^{-})] \le E[\overline{V}(x^{-})] = \Pr[f(x^{-}) \ge f^{\equiv}]$. By symmetry, these probabilities are identical for all $x^{-} \in X^-$. As $E[f(x^{-})] = f^{-}$, $f^{\equiv} - f^{-} = \Theta(m / n)$, and $f(x) - f^{-} = \Theta(\lambdabound m / n)$, the Chernoff bound~\eqref{eq:chernoffvar} gives
\begin{align*}
\Pr[f(&x^{-}) \ge f^{\equiv}]= \Pr[f(x) - f(x^{-}) \le f(x) - f^{\equiv}] \\
    &= \Pr[f(x) - f(x^{-}) \le f(x) - f^{-} + f^{-} - f^{\equiv}] \\
    &= \Pr\left[f(x) - f(x^{-}) \le E[f(x) - f(x^{-})] - \Theta(m/n)\right] \\
    &\le \max\{\exp(-\Theta(m^2/n^2) / (4 (3\lambda/n) m)), \exp(-(3/8) \Theta(m/n))\}\\
    &= \max\{\exp(-\Theta(m/\lambda n)), \exp(-\Theta(m/n))\}\\
    &= \exp(-\Theta(m/\lambda n)).
\end{align*}
Note that $f(x) - f(x^{-})$ is the sum of $m$ independent random variables describing the influence of each of the $m$ random clauses on this expression. With probability at least $1-3\lambda/n$, a random clause contains none of the $\lambda$ variables $x$ and $x^-$ differ in. In this case, the clause contributes equally to $f(x)$ and $f(x^-)$, hence zero to the difference.

From the above, we conclude that whenever $\lambdabound = o(m / n)$, the multiple $(1 - \lambdabound E[\tilde{V}^{\Sigma}] / |X^{-}|)$ in~\eqref{failure-prob-raw} is $1 - o(1)$. This condition is superseded with $\lambdabound = o((m / n)^{1/4})$ from the theorem statement, which means that~\eqref{failure-prob-raw} simplifies to:
\begin{equation*}
\Pr[x \text{ is not \emph{well-behaved} by first clause}] \le \exp\left(-\Omega\left(\frac{m}{\ell^2 \lambdaboundsq}\right)\right).
\end{equation*}
After applying $\ell = O(\lambdabound)$ and $\lambdabound = o((m / n)^4)$, we get that:
\begin{equation*}
\Pr[x \text{ is not \emph{well-behaved} by first clause}] \le e^{-\omega(n)}.
\end{equation*}

The probability of dissatisfying the two remaining clauses is proven in the same way (actually, these statements will bring the sharper bounds). The union bound on not being \emph{well-behaved}, using all three clauses, is still $e^{-\omega(n)}$.

The probability of \emph{all} $x$ to be \emph{well-behaved} is thus still $1 - e^{-\omega(n)}$, as there are $2^n$ possible assignments, and after using union bound, the failure probability is at most $2^n \cdot e^{-\omega(n)} = e^{-\omega(n)}$. This means that, during the entire run, the $\onell$ EA, during the mutation phase, will choose a \emph{good} or \emph{excellent} offspring with the sample probability as it would do on \textsc{OneMax}, multiplied by a constant.

% the derivative is negative if ex > 1. to be done in journal version
With probability of at least $1 - (1 - 1 / (e\ell))^{\ell} \ge 1 - (1 - 1 / (e\lambdabound))^{\lambdabound} \ge 1 - e^{-1/e}$, one of the missing bits from the parent,
which is found in the chosen \emph{good} or \emph{excellent} offspring, will
get recombined with the parent and thus will produce an assignment which is one bit closer to the optimum. By Lemma~\ref{lemma-one-bit-flip-is-ok}, whose conditions are either covered by the conditions of this theorem or follow from the one-bit difference, this new assignment will be selected to the next generation.
\end{proof}

